Heavy Traffic Approximation of Equilibria in Resource Sharing Games

We consider a model of priced resource sharing that combines both queueing behavior and strategic behavior. We study a priority service model where a single server allocates its capacity to agents in proportion to their payment to the system, and users from different classes act to minimize the sum of their cost for processing delay and payment. As the exact processing time of this system is hard to compute, we introduce the notion of heavy traffic equilibrium as an approximation of the Nash equilibrium, derived by considering the asymptotic regime where the system load approaches capacity. We discuss efficiency and revenue, and in particular provide a bound for the price of anarchy of the heavy traffic equilibrium.

==> 4_classlevel.tex <==



\section{Heavy Traffic Approximation: Class Level}
\label{sec:classlevel}

Based on the heavy traffic processing time approximation results in
Theorem~\ref{thm:heavy}, one can also propose a similar heavy traffic
equilibrium (HTE) concept for class level games. However, although the
processing time approximation allows us to greatly simplify the
computation of best response strategies, we are not able to obtain a
closed form expression for the class level HTE.  
More specifically, we consider the heavy traffic approximation of the waiting time and define
$W_i^{HT}(\boldsymbol{\beta})=\left[(1-\rho)\mu\beta\gamma_i(\boldsymbol{\beta})\right]^{-1}$.
It then follows from 
Theorem~\ref{thm:heavy}
%Theorem~4
and Little's law that
\[
\lim_{\rho\rightarrow1}(1-\rho)W_i(\bsy{\beta})=\lim_{\rho\rightarrow1}\frac{\bE[N_i]}{\lambda_i}=\frac{1}{\lambda\beta_i\gamma(\bsy{\beta})}.
\]
Therefore $W^{HT}$ is asymptotically exact: as $\rho\rightarrow1$,
\[
(1-\rho)[W^{HT}_i(\bsy{\beta})-W_i(\bsy{\beta})] \rightarrow 0.
\]
Similarly, we can define $\boldsymbol{\beta} =
(\beta_1, \cdots, \beta_K)$ as a class level heavy traffic equilibrium if
\begin{align*}
\beta_i&=\arg\min_{\beta>0}~c_iW_i^{HT}(\beta_1, \cdots , \beta_{i-1}, \beta, \beta_{i+1}, \cdots, \beta_K)+\beta^{\alpha}\\
&=\arg\min_{\beta>0}~\frac{c_i}{(1-\rho)\mu\beta\gamma_{-i}(\beta; \boldsymbol{\beta})}+\beta^{\alpha},
\end{align*}
for all $i = 1, \cdots, K,$ where
\[
\gamma_{-i}(\beta; \boldsymbol{\beta})=\frac{1}{\rho}\left[\sum_{j=1,j\neq i}^K\frac{\rho_j}{\beta_j}+\frac{\rho_i}{\beta}\right].
\]

We can obtain a system of {\em non-linear} equations to compute this class level heavy traffic equilibrium, 
but we are not able to get any closed form expressions for it, 
mainly due to two features of $\gamma_{-i}(\beta; \bsy{\beta})$ 
that are different from $\gamma(\boldsymbol{\beta})$ of a job level game. 
First, $\gamma_{-i}(\beta; \bsy{\beta})$ is subscripted by $i$, which implies that different classes face 
different environments in the system. 
This is because, unlike the infinitesimal single user in job level problem, 
each class as a player is not negligible in the system. 
Second, $\gamma_{-i}(\beta; \bsy{\beta})$ explicitly depends on $\beta$, the action of class $i$,
due to the {\em intra-class externality} behavior: 
in a class level game, a class chooses one
priority level for {\em all} its jobs simultaneously; 
while in a job level game, a job can choose any priority level regardless of other jobs belonging to its class.


Nevertheless, the intra-class externality effect will
become negligible in a regime where the number of classes is large;
this is a particularly useful regime for computing services where the
number of users grows large, and each user is viewed as a
distinct class. This observation motivates us to consider
a limiting model in which the number of classes approaches infinity
and any single class becomes infinitesimal. Thus, it can be connected
to the job level game model. We show that in the large system
limit of the class level game,
the heavy traffic equilibrium exists, is unique, can be computed in closed form,
and is the limit of the finite class equilibrium as the number of
class goes to infinity. Detailed discussions and proofs are in the Appendix H.
%%%We refer the reader to the
%%%companion technical report for an investigation of this
%%%limiting class level game model in which we show that the heavy
%%%traffic equilibrium exists, is unique, can be computed in closed form,
%%%and is the limit of the finite class equilibrium as the number of
%%%class goes to infinity \cite{techreport}


%Although the heavy traffic processing time approximation $V^{HT}$ proves to be asymptotically exact
%and the job level heavy traffic equilibrium it induces has closed form solution,
%we cannot simply repeat this in the class level game.
%The aggregate processing time is
%inspired by a ``one-versus-many'' view that is rigorously justified in
%a heavy traffic regime: a single job has little impact
%on the whole system when the system is sufficiently loaded.  By
%contrast, the same is not true in a class level model: even if the
%load increases, a single class amounts to a constant fraction of jobs
%in the system, so the equivalent aggregate priority as seen by one
%class will differ from the aggregate priority as seen by another
%class. In other words, the main difference between job level and class level
%equilibrium is the {\em externality} within a class.
%While a job can choose any priority level regardless of other jobs in
%that class in the job level game, the class chooses one
%priority level for {\em all} its jobs simultaneously in the class level game.
%
%To make progress, recall that our main interest in the class level
%model comes from the view that a single {\em user} of a resource
%sharing service corresponds to an entire class, i.e., that this user
%generates multiple jobs and chooses a single priority level for her
%entire family of jobs.  We note that for resource sharing
%services, a regime of particular interest is one where the number of
%users is large.  In our context, therefore, we are led to consider a
%regime where the number of {\em classes} is large.
%We refer the readers to the Appendix~B for a limiting model
%where the number of classes approaches infinity and any single class becomes infinitesimal.
%We define the heavy traffic equilibrium in the limit case, 
%which is unique, asymptotically exact, and exactly the limit of finite class model.

% In particular, fix a class $i$, we can assume jobs from
% this class are processed with a single class with priority
% $\hat{\beta}_i$ that is equivalent to all other classes, and then
% compute $W_1(\beta_i, \hat{\beta}_i)$ through
% (\ref{eq:wtime2}). However, while  Hence, unlike the job level
% setting in which the aggregate priority $\hat{\beta}$ can be
% independent of the job that we are considering and excluded from the
% system, the aggregate priority of class $i$, $\hat{\beta}_i$, has to
% depend on $i$.  Then instead of having only one consistency condition
% and one unknown $\hat{\beta}$ in the job level games, there are $K$
% equations and $K$ unknowns $(\hat{\beta}_1, \cdots, \hat{\beta}_K)$
% involved in the consistency condition of class level games, leading to
% another intractability.

% Therefore, to overcome the
% difficulty of computing class level equilibrium, we may need to
% eliminate, or at least greatly reduce this externality within a
% class and make a class-level decision acting like a job-level
% decision.



